Why are Adaptive Methods Good for Attention Models?

While stochastic gradient descent (SGD) is still the \emph{de facto} algorithm in deep learning, adaptive methods like Clipped SGD/Adam have been observed to outperform SGD across important tasks, such as attention models. The settings under which SGD performs poorly in comparison to adaptive methods are not well understood yet. In this paper, we provide empirical and theoretical evidence that a heavy-tailed distribution of the noise in stochastic gradients is one cause of SGD's poor performance. We provide the first tight upper and lower convergence bounds for adaptive gradient methods under heavy-tailed noise. Further, we demonstrate how gradient clipping plays a key role in addressing heavy-tailed gradient noise. Subsequently, we show how clipping can be applied in practice by developing an \emph{adaptive} coordinate-wise clipping algorithm (ACClip) and demonstrate its superior performance on BERT pretraining and finetuning tasks.

==> sections/acclip.tex <==



\section{Gradient based optimization algorithms}\label{sec:algorithms}
	\vspace{-0.20cm}

Our key idea is that by \emph{clipping} the stochastic gradient, we can effectively control its variance. While this does introduce some additional bias, the clipping threshold can be (possibly adaptively) tuned to trade-off variance with the introduced bias. 
% Given that SGD does not converge when the stochastic gradient has unbounded variance, we propose clipped GD as a solution based on two intuitions: theoretically, the trimmed mean estimator is known to be robust against heavy-tailed noise; empirically, clipping is a common technique in noisy neural network training. Clipped gradient descent is provable convergent by analysis in Section~\ref{sec:thm}. We will now introduce two natural choices for clipping, global clipping and coordinate-wise clipping and compare them in details below.

Empirically, this is a prevalent practice e.g. \cite{merity2018regularizing} use clipped SGD to train AWD-LSTM whereas \cite{devlin2018bert} use clipped Adam to pretrain BERT. The general form of clipped gradient descent is outlined in Algorithm \ref{alg:general-clippedGD}.
\begin{algorithm}[H] 
    \caption{A general framework for clipped gradient descent}\label{alg:general-clippedGD}
	\begin{algorithmic}[1]
	    \State $x, m_k \gets x_0, 0$
	    \For {$k = 1, \cdot, T$}
	    \State $m_k \gets \beta_1 m_{k-1} + (1-\beta_1) g_k $
	    \State $\hat{g}_k \gets \clip(\tau_k, m_k)$
		\State $x_k \gets x_{k-1} - \eta_k \hat{g}_k$
		\EndFor
		\Return $x_K$, where random variable $K$ is supported on $\{1, \cdots, T\}$.
	\end{algorithmic}\vspace{-0.1cm}
\end{algorithm}

Perhaps the two most natural candidates for clipping mechanisms are {Global~CLIPping} where a single global threshold is used and {Coordinate-wise~CLIPping} using $d$ coordinate-wise thresholds
\begin{align}
    \text{GClip}(\tau_k, m_k) &= \min\cbr[\big]{\tfrac{\tau_k}{\|m_k\|}, 1}m_k\,, \text{ for } \tau_k \in \mathbb{R}_{\geq 0} \text{ or,} \label{eqn:g-clip}\tag{GClip}\\
    \text{CClip}(\tau_k, m_k) &= \min\cbr[\big]{\tfrac{\tau_k}{|m_k|}, 1}  m_k\,, \text{ for } \tau_k \in \mathbb{R}_{\geq 0}^d\,. \label{eqn:c-clip}\tag{CClip}
\end{align}
where all operations for CClip are performed element-wise. Smaller threshold values of $\tau_k$ imply smaller variance, but also higher bias. 
If the noise distribution is very heavy-tailed (or has a large variance), one could compensate by picking a smaller threshold. See Theorems~\ref{thm:strongly-convex-convergence}~and~\ref{thm:nonconvex-convex-convergence} for a theoretical treatment of this for GClip.
While GClip preserves the update direction and only scales its magnitude, CClip scales each coordinate individually and may not preserve the direction. However, if the noise distribution varies significantly across coordinates, CClip can take advantage of this and only clip those which are more heavy-tailed and consequently converge faster (see Theorem~\ref{thm:c-clip-convergence}).

However, to perform such a coordinate-wise variance-bias trade off optimally would require tuning all $d$ thresholds, which could be extremely large in deep learning. Even if tuning were feasible, the noise distribution may be non-stationary and significantly vary as training progresses (see Fig.~\ref{fig:nonstationary}). To address this challenge, we propose Adaptive Coordinate-wise CLIPping, which \emph{adaptively} sets the thresholds for each coordinate
\begin{align*}\label{eqn:acc-clip}
    \text{ACClip}(\tau_k, m_k) = \min\cbr[\big]{\tfrac{\tau_k}{|m_k|+\epsilon}, 1}m_k,\quad 
    \tau_k^\alpha = \beta_2 \tau_{k-1}^\alpha + (1 - \beta_2) |g_k|^\alpha\,, \tag{ACClip}
\end{align*}
where operations are element-wise, $\epsilon$ is a small number for numerical stability, and we set $\alpha=1$ by default. The use of a coordinate-wise $\alpha$-moment (as opposed to the traditional second moment) is motivated by our theory and estimates $B = \E[|g_k^\alpha|]^{1/\alpha}$ in Assumption~\ref{assump:coord-noise}. Since $\E[|g_k^\alpha|]^{1/\alpha}$ is increasing in $\alpha \geq 1$, using $\alpha =1$ is a conservative bound on $B$ when the true $\alpha$ is unknown. 
%Interestingly, Adam can also be viewed as performing adaptive coordinate-wise clipping.
% Not surprisingly Adam, which also performs such empirical moment estimates and can be seen to perform an ad-hoc clipping, is closely related.
% The key difference is that our algorithm increases the clipping threshold as the step size decreases whereas Adam does not. The increasing threshold will reduce the bias in the gradient estimator and leads to accelerating the empirical convergence as shown in Section~\ref{sec:experiment}.

% Global clipping is a common technique used on top of the gradient-based optimizer. In AWD-LSTM~\citep{merity2018regularizing},  global clipping is used on top of SGD. In BERT~\citep{devlin2018bert} pretraining, global clipping is applied on Adam. Intuitively, clipping prevents the heavy tailed noise from dragging the current solution to an unstable region by controlling the distance moved. The convergence of globally clipped gradient descent is proven in Section~\ref{sec:thm}.

% However, as later shown in Figure~\ref{fig:loss-curves-bert}, the empirical performance of clipped SGD with momentum could be much worse than Adam. Motivated by this finding, we study the following coordinate-wise clipped gradient descent algorithm, which is closely related to Adam when $\beta_1 = 0$ (i.e. RMSProp) as shown in Section~\ref{sec:RMSProp}.

% \textbf{Coordinate-wise clipped gradient descent} with a vector clipping parameters $\tau_k \in \mathbb{R}^d$ can be written as 
% All the operators above are \textit{elementment-wise} when applied to two vectors. we prove the convergence of coordinate-wise clipped gradient descent in Thm~\ref{thm:nonconvex-cclip}. On a high level, we show that when the noise distributes very differently across different coordinate, then CClip can have better dimension dependence compared to GClip.

% Based on the proof for cooridnate-wise clipping, we found that the clipping threshold $\tau_k$ for coordinate-wise clipped gradient descent should scale linearly with $B/\eta_k$, where $\eta_k$ is the step size and $B$ is defined in Assumption~\ref{assump:coord-noise}. From this result, and the fact that the noise distribution is nonstationary (see Figure~\ref{fig:nonstationary}) throughout training, we propose the \textbf{adaptive coordinate-wise clipped gradient descent} (ACClip) algorithm. It estimate the value $B_i$ defined in Assumption~\ref{assump:coord-noise} by an exponential moving average as follows
% \begin{align*}\label{eqn:acc-clip}
%     \clip(\tau_k, m_k) = \min\cbr[\big]{\tfrac{\tau_k^{(i)}}{|m_k|+\epsilon}, 1}m_k,\quad 
%     \tau_k = \beta_2 \tau_{k-1} + (1 - \beta_2) |g_k|. \tag{ACClip}
% \end{align*}

% $\epsilon$ is a small number to avoid numerical instability. As before, the operators when applied to vectors are defined as element-wise operation. In the next subsection, we will show that Adam is closely related to our proposed algorithm. The key difference is that our algorithm increases the clipping threshold as the step size decreases, which in Adam corresponds to increasing $\beta_2$ as the step size decreases. The increasing threshold will reduce the bias in the gradient estimator and leads to accelerating the empirical convergence as shown in Section~\ref{sec:experiment}.


% If we assume the estimator approximates $\E[\|g_k\|^2]^{1/2}$ within constant factor and is further a good approximation of $\E[\|g_k\|^\alpha]^{1/\alpha}$, then Adam converges if the step size approahces 0 and $\beta_2$ approaches $1$.

 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../root"
%%% End:

